Access Management in Joint Sensing and Communication Systems: Efficiency versus Fairness

In this paper, we consider a distributed joint sensing and communication (DJSC) system in which multiple radar sensors are deployed. Each sensor is equipped with a sensing function and a communication function, and thus it is a JSC node. The JSC nodes are able to perform sensing their surrounding environments, e.g., weather conditions or available spectrum. Furthermore, they can cooperatively detect and track a common target. The information, i.e., of the environment and target, collected by the JSC nodes is transmitted to a base station (BS) for further processing. As such, different aspects of the target to be viewed simultaneously, which significantly improves the performance of the target detection and tracking. However, both the sensing function and communication function require a certain amount of bandwidth for their operations, and deploying multiple JSC nodes may consume a large amount of bandwidth. Therefore, we investigate the bandwidth allocation problem for the DJSC system. In particular, we aim to optimize the bandwidth allocation to the sensing function and the communication function of the JSC nodes. To improve the allocation efficiency while benefiting the spatial diversity advantage of the DJSC systems, the objective is to maximize the sum of sensing performances, i.e., estimation rates, communication performances, i.e., communication data rates, and fairnesses of all the users. The optimization problem is non-convex and difficult to be solved. For this, we propose a fully polynomial time approximation algorithm, and we prove that the approximation algorithm can guarantee a near-optimal solution with an accuracy bound of $\epsilon$. Furthermore, we propose to use a heuristic algorithm with lower complexity. The simulation results show that both the proposed algorithms are able to achieve the solutions close to the optimum in a computationally efficient fashion.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> discrete.tex <==
\subsection{Approximation algorithm for the discrete case}
\label{sec:ptas-integer}
In this section, we assume that variables $B_i^C$ and $B_i^R$ assume integer values, and hence the utility functions are discrete. By scaling if necessary, we may also assume that all the utilities are at least 1. We will present a polynomial time algorithm that can produce a near-optimal solution to the problem FSA with a theoretical guarantee on the quality of the solution. In fact, we will show the following result.
\begin{theorem}
\label{thm:app-sche}
For any given constant $\epsilon\in(0,1]$ one can compute in polynomial time a solution to the problem FSA, whose value is within a factor of $1-\epsilon$ of the optimal value. The running time of the algorithm is $O(N^3(\frac{1}{\epsilon^2}+\log(N\max_{i=1}^nu_i(B)))$
\end{theorem}

In \cite{AgraliG09} Agrali and Geunes designed an FPTAS for the problem in the absence of the constraint (\ref{const:lu-bound}). In this work we aim to develop a more efficient DP-based FPTAS that not only can handle this constraint but also  have a better running time. In fact, the complexity of our algorithm is upper bounded by $O(N^3(\frac{1}{\epsilon^2}+\log \Gamma))$, compared to $O(N^5(\frac{1}{\epsilon^2}+\log \Gamma))$ obtained in  \cite{AgraliG09}, where $\Gamma=\max_{i\in [N]} u_i(B)$.

{\em A high level description of the algorithm.} We first present a dynamic programming-based algorithm for solving exactly the problem, whose running time is pseudo-polynomial time in the size of the problem instance. We then use this algorithm as a sub routine in order to obtain an $(1-\epsilon)$-approximation algorithm as desired. Without loss of generality, one can assume that $\epsilon$ is a rational number.

Since we will make use of the dynamic programming in terms of utilities, it is needed that all the radar and the communicate functions take integer value for any given integer input. This is, however, not the case in our model. To solve this issue, we first round down the functions
as
\[
R_{i}^{\text{C}}= (1+\epsilon)^{\lfloor \log_{1+\epsilon} R_{i}^{\text{C}} \rfloor}, \quad R_{i}^{\text{R}}= (1+\epsilon)^{\lfloor \log_{1+\epsilon} R_{i}^{\text{R}} \rfloor}
\]
for all $i\in[N]$, and then use a scaling approach. One can show that this procedure can reduce the optimal value of FSA by a factor of $1+\epsilon$. 

Note that the possible values for each variable (which are assumed to be integers) can be {\it exponentially} large in the input size. Thus, we need also to round this set of possible values so that their total number is polynomial in $\log\Gamma$. Utilizing the monotonicity of the functions $R_i^C(\cdot)$ and $R_i^R(\cdot)$), this can be achieved again by restricting each variable $B_i^C$ (resp, $B_i^R$) to values at which the functions $R_i^C(B_i^C)$ (resp., $R_i^R(B_i^R)$) increase by a  factor of $1+\epsilon$, losing only an additional factor of $(1+\epsilon)$ in the overall approximation ratio.

In the following we will first  consider the simplified problem FSA' instead of FSA, in which the integer-value version of radar and communication functions are considered. 

  
\begin{lemma}
There is a pseudo-polynomial time algorithm for solving FSA with integer variables, whose running time is $O(N\Gamma^2)$.
\end{lemma}  
  \begin{proof}
 Let $\cI$ be an instance problem of  FSA'.  We first fix some notations used in the description of our DP algorithm. By the rounding and scaling aforementioned it holds that $u_i(B_i)\ge 1$ for $B_i\ge 1$. For the case when $B_i>\xi_i$ we set $u_i(B_i)=-\infty$, without affecting the optimal objective value. For a given {\em feasible} (partial) allocation $\cB^\ell=(B_{1}, \ldots, B_{\ell})$, where $K\le N$, define $\mu(\cB^\ell)=\sum_{i=1}^K B_{i}$ to be the size of $\cB$. Here the feasibility means that the allocation satisfies the constraint (\ref{const:lu-bound}). Note that the objective  value w.r.t $\cB$ is given by 
 \[
 \Phi(\cB^\ell) = {\sum}_{i\in [\ell]}u_i(B_i).
 \]
  For each $\ell\in[N]$ and a nonnegative integer $p$, let $\cA[\ell, p]$ denote the smallest size of an allocation $\cB$ among the first $\ell$ users such that $\Phi(\cB^\ell) =p$. Formally,
\begin{equation}
\label{eq:alp}
\cA[\ell, p] = \min \left\{\mu(\cB^\ell)~|~\Phi(\cB^\ell)=p\right\}.
\end{equation}  
   Let $\cB^{\ell,p}$ be  the allocation corresponding to $\cA[\ell,p]$. It is further noticed that for a user $i$ who is allocated a bandwidth $B_i$, one can show later that the value  $u_i(B_i) $ determined by (\ref{utility_user}) can be found efficiently.  
An upper bound $\Gamma$ on the value of an optimal solution can be taken as $\Gamma=\sum_{i\in[N]}u_i(B)$.

\vspace{5pt}

{\bf DP Algorithm:}
\begin{itemize}
\item Input: $\{R_i^{\text{C}},R_i^{\text{R}}\}_{i\in[N]},B,\Gamma$
\item Initial step: $\cA[0, 0] \leftarrow  0, \cA[0, p] \leftarrow  B+1$ for $p \in[\Gamma]$
\item Recursive step: For $i\in[N]$, compute $\cA[\ell,p]$ as the optimal value of the following problem:
\[
\min_{\underline \xi_i\le B_{i}\le \overline \xi_i,u_i(B_i)\le p} \left \{\cA[i - 1, p - u_i(B_i)]\right\}
\]
for each $p\in \{0\}\cup [\Gamma]$.
\item Output: $\cB^*\leftarrow \text{argmax} \{\cB^{N, p}~|~ \cA[N,p] \le B\} $
\end{itemize}

{\em Correctness and complexity of DP.} 
It is easy to see that the correctness of the recurrence relation follows immediately from the definition of $\cA[\ell,p]$ in (\ref{eq:alp}). To show the running time of DP, note that the dominant phase is the recursive step which is repeated $N$ times. Furthermore, each iteration in this step is carried out in $O(\Gamma^2)$, since $0\le p  \le \Gamma$ and only the (nondominated) values of $B_i$ are considered, as the function $u_i(B_i)$ is strictly increasing. Consequently,  the overall complexity of the algorithm is upper bounded by $O( N\Gamma^2)$.
\end{proof}

We now give a proof  of Theorem \ref{thm:app-sche} by presenting a polynomial-time algorithm, as shown in Algorithm \ref{fptas}. Essentially, we will try to apply the DP algorithm with an upper bound of $\Omega=4N$, instead of $\Gamma$, to solve a number of scaled problem instances until the value of an optimal allocation $\cB^*$ is at least some fixed bound. This will be done after a finite number of steps, lets say $\bar k$, and the value $\Phi(\cB^*)$ belongs to the interval $(2^{\bar k}, 2^{\bar k+2)}]$.  In Step~\ref{solution} of Algorithm \ref{fptas}, the DP algorithm  is used again with an upper bound of $\Omega=\lceil (1+\frac{3}{\epsilon})N\rceil$ to solve a new scaled instance to return a solution which is close to the optimum of the original instance $\cI$ of  FSA'. 
%Finally, both phases use a lower bound $L$ on the utility $\bF_+(x^*)$. Here we simply take $L = \max_{i=1}^n\{u_i(B)\}.$


\begin{algorithm}[!htb]
	\caption{{\bf FPTAS}$(\{u_i\}_{i\in[N]},B,\epsilon)$} \label{fptas}
\begin{algorithmic}[1]
\Require Utility functions $u_i$, $i\in[N]$, the bandwidth capacity $B$, and an accuracy parameter $\epsilon>0$
\Ensure A solution $\hat \cB$
\State $\Gamma\leftarrow\sum_{i=1}^Nu_i(B)$, $k \leftarrow  \left\lceil\log_2  \Gamma\right\rceil$
%\Repeat 
%\label{loop}
\State For each $i\in[N]$ define 
$\widetilde{u_i}(B_i)\leftarrow \left\lfloor u_i(B_i)\cdot (N/2^k)\right\rfloor$\label{step:scale}
\State Run the DP algorithm with $(\{\widetilde u_i\}_{i\in[N]},B,4N)$ as input and let $\widetilde \cB$ be the returned solution.
\label{dyn}
\State If $\sum_{i=1}^N\widetilde u_i(\widetilde B_i)\ge N$ then break; otherwise set $k\leftarrow k-1$;\label{halt}
\State If $k>0$ then go back Step \ref{step:scale}  \label{kvalue}
%\Until $k=0$
%\label{kvalue}
\State For each $i\in[N]$ define  $\widetilde{u_i}(B_i)\leftarrow \left\lfloor u_i(B_i)\cdot (\epsilon N/2^k)\right\rfloor$
\State Run the DP algorithm with $(\{\widetilde u_i\}_{i\in[N]},B,\lceil (1+\frac{3}{\epsilon})N\rceil)$ as input and let $\hat \cB$ be the returned solution. 
\label{solution}
\State \Return $\hat \cB$
\end{algorithmic}
\end{algorithm}


We show that the  termination condition at Step~4 holds for some value of $k$. To this end, we partition the interval $(1, \Gamma]$  into $\left\lceil\log_2  \Gamma\right\rceil$ disjoint intervals 
\[
[1, \Gamma)={\bigcup}_{k=1}^{\left\lceil\log_2  \Gamma\right\rceil}[2^{k-1},2^k).
\]
Since $\Phi(\cB^*)\le \Gamma$, there must be a value of $k$, say $k'$, such that $\Phi(\cB^*)$ belongs to the interval $[2^{k'}, 2^{k'+1})$. It follows that
\begin{equation}
4N> \dfrac{N\cdot \Phi(\cB^*)}{2^{k'-1}}\ge N \Rightarrow 
4N>\left\lfloor \dfrac{N\cdot\Phi(\cB^*)}{2^{k'-1}}\right\rfloor\ge N.
\label{eq:1}
\end{equation}
%since $\Phi(\cB^*)\ge 2^{k'}$. 

The Eq. (\ref{eq:1}) implies that $\cB^*$ is satisfied by the termination  condition at Step  \ref{halt}, with the corresponding value $k = k'-1$. We next bound the value of $\cB^*$ as in the following lemma.
\begin{lemma}
\label{lem:lu-bound}
Let $\bar k$ be the value of $k$ after Step \ref{kvalue} of Algorithm \ref{fptas}. Thenwe must have that $2^{\bar k}\le \Phi(\cB^*)< 3.2^{\bar k}$.% \le 2(2^{\bar k-1})(LB)$.
\end{lemma}
\begin{proof}
The Eq. (\ref{eq:1}) implies that 
\[
N>\left\lfloor  \dfrac{N\cdot\Phi(\cB^*)}{2^{\bar k+1}}\right\rfloor > \dfrac{N\cdot\Phi(\cB^*)}{2^{\bar k+1}}-1.
\] 
and thus,
 \begin{equation}
 \label{eq:2}
\Phi(\cB^*)<\dfrac{N+1}{N}\cdot 2^{\bar k+1}<3\cdot 2^{\bar k},
\end{equation}
for  $N\ge 2$.

It remains to show the lower bound of $\Phi(\cB^*)$. 
Denote by $\widetilde \cB$ the allocation returned by Algorithm \ref{fptas} for $k =\bar k$. Then, $\widetilde \cB$ fulfills the halt condition at Step \ref{halt}, i.e.,
\begin{equation}
\label{eq:3}
 {\sum}_{i=1}^N \left\lfloor \dfrac{N\cdot u_i(\widetilde B_i)}{2^{k'}}\right\rfloor \ge N.
\end{equation}
Moreover, since $\cB^*$ is the optimal allocation to $\cI$, it follows that:
\begin{align}
\label{eq:4}
\Phi(\cB^*)\ge \Phi(\widetilde \cB)=&~\sum_{i=1}^N u_i(\widetilde B_i)\nonumber\\
\ge&~ \dfrac{2^{\bar k}}{N}\left( \sum_{i=1}^N \left\lfloor \dfrac{N\cdot u_i(\widetilde B_i)}{2^{k'}}\right\rfloor \right).
\end{align}
From (\ref{eq:3}) and (\ref{eq:4}), we have that
%\begin{equation}
%\label{eq:5}
$\Phi(\cB^*)\ge2^{\bar k}$, and this 
%\end{equation}
  completes the proof.
\end{proof}


%\begin{theorem} 
%\label{th:fptas}For any constant $\epsilon>0$, Algorithm \ref{fptas} runs in time $O(N^3(\frac{1}{\epsilon^2}+\log(N\max_{i=1}^nu_i(B)))$ and produces a $(1-\epsilon)$-approximate solution $\hat \cB$ to the  instance $\cI $. 
%\end{theorem}
We are now ready to prove Theorem \ref{thm:app-sche}. Suppose that Algorithm \ref{fptas} outputs an allocation $\hat \cB$. We prove that $\Phi(\hat \cB)\ge  (1-\epsilon)\cdot \Phi(\cB^*)$. We first argue that there is an allocation returned after Step \ref{solution} of Algorithm \ref{fptas}. To prove this, note that 
\begin{align*}
\sum_{i=1}^N \left\lceil \dfrac{N\cdot u_i( B^*_i)}{\epsilon  2^{\bar k}}\right\rceil \le &~
\left\lceil \dfrac{N\cdot \sum_{i=1}^N u_i( B^*_i)}{\epsilon  2^{\bar k}}+N\right\rceil \\
=&~ \left\lceil \dfrac{N\cdot \Phi(\cB^*)}{\epsilon  2^{\bar k}}+N\right\rceil
< \left\lceil \left(1+\dfrac{3}{\epsilon}N\right)\right\rceil.
\end{align*}
Therefore, $\cB^*$ is an allocation to the instance $(\{\widetilde u_i\}_{i\in[N]},B)$, whose  value is at most $\lceil (1+\frac{3}{\epsilon}N\rceil$. The last inequality above is due to Eq.  (\ref{eq:2}).

We have that 
\begin{align*}
\Phi(\hat \cB)& \,\,=\sum_{i=1}^N u_i(\hat B_i)\ge \dfrac{\epsilon 2^{\bar k}}{N}\left( \sum_{i=1}^N \left\lceil \dfrac{N\cdot u_i(\hat B_i)}{\epsilon  2^{\bar k}}\right\rceil -N \right)\\
& \,\,\ge \dfrac{\epsilon 2^{\bar k}}{N}\left( \sum_{i=1}^N \left\lceil \dfrac{N\cdot u_i( x^*_i)}{\epsilon  2^{\bar k}}\right\rceil -N \right)\\
& \,\,\ge \dfrac{\epsilon 2^{\bar k}}{N}\left( \dfrac{N\cdot\Phi(\cB^*)}{\epsilon  2^{\bar k}} -N \right)\\
& \,\, = \Phi(\cB^*)-\epsilon 2^{\bar k}\ge (1-\epsilon)\cdot \Phi(\cB^*).
\end{align*}
The third inequality is due to the fact that $\hat \cB$ is the best allocation  to the instance $(\{\widetilde u_i\}_{i\in[N]},B)$, among the ones whose value is bounded by $\lceil (1+\frac{3}{\epsilon})N\rceil$. The last inequality comes from Lemma~(\ref{lem:lu-bound}).

Regarding the complexity part,  the running time of Algorithm \ref{fptas} is $O(T+V)$, where $T$ is the amount of time needed to solve a sequence of scaled instances until the termination condition at Step~4 hold, and $V$ is the amount of time needed for solving anther instance at Step \ref{solution}. Firstly, since we run the DP algorithm for  scaled instances, each with upper bound $4n$ at Step \ref{dyn}, it follows that $T=O(N^3\left\lceil \log_2 \Gamma\right\rceil)$. Secondly, finding an allocation at Step \ref{solution} takes  $V=O(N^3/\epsilon^2)$ times as the bound of $\lceil (1+\frac{3}{\epsilon})N\rceil$ is used in the DP algorithm in this step. Hence, the overall  running time of Algorithm \ref{fptas} is  $O(N^3(\frac{1}{\epsilon^2}+\log(\Gamma))$. This completes the proof.


==> kkt_reduction.tex <==
Define the Lagrangian function:
\begin{align*}
& \mathcal{L}=  \sum_{i=1}^N (f_i(x_i^{\text{R}})+g_i(x_i^{\text{C}}))+\alpha (B-\sum_{i=1}^N (x_i^{\text{R}}+x_i^{\text{C}}))\\
+& \mu^T x + \sum_{i=1}^N \lambda_i (\overline\xi_i - x_i^{\text{R}}-x_i^{\text{C}}) - \sum_{i=1}^N \eta_i (\underline\xi_i - x_i^{\text{R}}-x_i^{\text{C}}),
\end{align*}
where $\alpha, \mathbf {\mu, \eta, \lambda}$ are Lagrange multipliers.

By the Karush-Kuhn-Tucker necessary conditions for an optimal solution \cite{LY15}, we must have that:

\begin{itemize}
\item {\em Stationarity of the Lagrangian:}
\begin{align}
\mathcal{L}'_{ x_i^{\text{R}}} = f'_i(x_i^{\text{R}}) -\alpha+\mu_i^{\text{R}} -\lambda_i  +\eta_i=0\label{dependR}\\
\mathcal{L}'_{ x_i^{\text{C}}} = g'_i(x_i^{\text{C}}) -\alpha+\mu_i^{\text{C}} -\lambda_i  +\eta_i=0\label{dependC}
\end{align}
for each $i\in[N]$.
\item {\em Complementarity conditions:}
\begin{align}
\alpha (B-{\sum}_{i=1}^N (x_i^{\text{R}}+x_i^{\text{C}})) = & ~0\label{resource-constraint}\\
\mu_i^{\text{R}} x_i^{\text{R}}=&~0\label{xiR}\\
\mu_i^{\text{C}} x_i^{\text{C}}=&~0\label{xiC}\\
\lambda_i (\overline\xi_i - x_i^{\text{R}}-x_i^{\text{C}}) = &~0\label{xiRC1}\\
\eta_i (\underline\xi_i - x_i^{\text{R}}-x_i^{\text{C}}) = &~ 0.\label{xiRC2}
\end{align}
for each $i\in[N]$.
\item {\em Primal feasibility of the solution:}
\begin{align}
B\ge~& {\sum}_{i=1}^N (x_i^{\text{R}}+x_i^{\text{C}})\\
\overline\xi_i \ge~& x_i^{\text{R}}+x_i^{\text{C}}\\
\underline\xi_i \le~& x_i^{\text{R}}+x_i^{\text{C}}
\end{align}
for each $i\in[N]$.
\item {\em Non-negativity of the multipliers:}
\begin{align}
\alpha\in\mathbb{R}_+,\mathbf {\mu} \in \mathbb{R}_+^{2N},\mathbf {\eta, \lambda} \in \mathbb{R}_+^{N}
\end{align}
Note that $\alpha>0$, since $f_i,g_i$ are increasing functions for every $i\in[N]$ and thus the constraint (\ref{resource-constraint}) should be active.
\end{itemize}
In what follows we show that the number of KKT points, i.e. the solutions of the system It follows from Eq. (\ref{xiR}) that
\begin{align}
x_i^{\text{R}}=0\quad \text{and}& \quad \mu_i^{\text{R}}\not=0, & \text {(I)}\label{xiRa}\\
\text{or}\quad  x_i^{\text{R}}\not=0\quad \text{and}& \quad \mu_i^{\text{R}}=0, & \text {(II)}\label{xiRb}
\end{align}
It follows from Eq. (\ref{xiC}) that
\begin{align}
x_i^{\text{C}}=0\quad \text{and}& \quad \mu_i^{\text{C}}\not=0, & \text {(III)}\label{xiRa}\\
\text{or}\quad  x_i^{\text{C}}\not=0\quad \text{and}& \quad \mu_i^{\text{C}}=0, & \text {(IV)}\label{xiRb}
\end{align}
From Eq. (\ref{xiRC1}) and (\ref{xiRC2}) we have:
\begin{align}
x_i^{\text{R}}+x_i^{\text{C}}=\overline\xi_i,\quad \text{and}& \quad \lambda_i\not=0, & \text {(V)} \label{xiRa}\\
x_i^{\text{R}}+x_i^{\text{C}}=\underline\xi_i,\quad \text{and}& \quad \eta_i\not=0, & \text {(VI)} \label{xiRa}\\
\underline\xi_i <x_i^{\text{R}}+x_i^{\text{C}}<\overline\xi_i,\quad \text{and}& \quad \lambda_i=\eta_i=0, & \text {(VII)}\label{xiRb}
\end{align}

Denote  $I_i=[\underline\xi_i,\overline\xi_i]$. Consider the following  cases 



\noindent{\bf Case 1: (I) $\wedge$ (IV) $\wedge$ (V)}. It follows that $x_i^{\text{R}}=0,x_i^{\text{C}}=\overline\xi_i$. Define $F^{(1)}_i(\alpha)=g_i(\overline\xi_i)$, and $G^{(1)}_i(\alpha)=\overline\xi_i$. %Note that in this case $\mu_i^{\text{C}}=\eta_i=0$ and from (\ref{dependC}) it follows that $\alpha+\lambda_i=g'_i(x_i^{\text{C}})\Rightarrow \alpha\le g'_i(\overline\xi_i)$.

\noindent{\bf Case 2: (II) $\wedge$ (III) $\wedge$ (V)}. It follows that $x_i^{\text{C}}=0,x_i^{\text{R}}=\overline\xi_i$. Define $F^{(2)}_i(\alpha)=f_i(\overline\xi_i)$, and $G^{(2)}_i(\alpha)=\overline\xi_i$. %Using the similar argument as in Case 2, we have $\alpha\le f'_i(\overline\xi_i)$.

\noindent{\bf Case 3: (I) $\wedge$ (IV) $\wedge$ (VI)}. It follows that $x_i^{\text{R}}=0,x_i^{\text{C}}=\underline\xi_i$. Define $F^{(3)}_i(\alpha)=g_i(\underline\xi_i)$, and $G^{(3)}_i(\alpha)=\underline\xi_i$. 

\noindent{\bf Case 4: (II) $\wedge$ (III) $\wedge$ (VI)}. It follows that $x_i^{\text{C}}=0,x_i^{\text{R}}=\underline\xi_i$. Define $F^{(4)}_i(\alpha)=f_i(\underline\xi_i)$, and $G^{(4)}_i(\alpha)=\underline\xi_i$.

\noindent{\bf Case 5: (II) $\wedge$ (IV) $\wedge$ (VI)}. It follows that $x_i^{\text{C}}\not=0,x_i^{\text{R}}\not=0$, and $x_i^{\text{R}}+x_i^{\text{C}}=\underline\xi_i$. Define $F^{(5)}_i(\alpha)=u_i(\underline\xi_i)$, and $G^{(5)}_i(\alpha)=\underline\xi_i$.


\noindent{\bf Case 6: (II) $\wedge$ (IV) $\wedge$ (V)}. It follows that $x_i^{\text{C}}\not=0,x_i^{\text{R}}\not=0$, and $x_i^{\text{R}}+x_i^{\text{C}}=\overline\xi_i$. Define $F^{(6)}_i(\alpha)=u_i(\overline\xi_i)$, and $G^{(6)}_i(\alpha)=\overline\xi_i$.

\noindent{\bf Case 7: (I) $\wedge$ (IV) $\wedge$ (VII)}. It follows that $x_i^{\text{R}}=0,x_i^{\text{C}}\in I_i$, and $\mu_i^{\text{C}}=\lambda_i=\eta_i=0$. Define 
\[
F^{(7)}_i(\alpha)=\left\{\begin{matrix}
g_i(g_i^*(\alpha))  & \text{if}\quad  g_i^*(\alpha)\in I_i\\ 
0 & \text{if} \quad  g_i^*(\alpha)\not\in I_i
\end{matrix}\right.
\]
and $G^{(7)}_i(\alpha)=g_i^*(\alpha)$. Note that $\alpha=g'_i(x_i^{\text{C}})\le g'_i(\underline\xi_i)$, as $g'_i$ is decreasing over $I_i$.

\noindent{\bf Case 8: (II) $\wedge$ (III) $\wedge$ (VII)}. It follows that $x_i^{\text{C}}=0,x_i^{\text{R}}\in I_i$, and $\mu_i^{\text{R}}=\lambda_i=\eta_i=0$. Since the radar function $f'_i$ is not a one-to-one mapping, one can define two possible pseudo inverse functions for this function as follows.
\[
f_i^{\downarrow}(\alpha)=\left\{\begin{matrix}
\frac{\frac{\delta}{T_p}+2\gamma_i\sqrt{(f'_i(\gamma_i))^2-\alpha^2}}{2\alpha} & \text{if}\quad &0<\alpha\le f'_i(\gamma_i)\\ 
0 & \text{if} \quad &\alpha>f'_i(\gamma_i)
\end{matrix}\right.
\]
and
\[
f_i^{\uparrow}(\alpha)=\left\{\begin{matrix}
\frac{\frac{\delta}{T_p}-2\gamma_i\sqrt{(f'_i(\gamma_i))^2-\alpha^2}}{2\alpha} & \text{if}\quad &0<\alpha\le f'_i(\gamma_i)\\
0 & \text{if} \quad &\alpha>f'_i(\gamma_i)
\end{matrix}\right.
\]
where $f'_i(\gamma_i)=f'_i(1/\sqrt{\gamma_i})=\frac{\delta\nu_i}{2T_p}$ is the maximum value of the function $f'_i$ on $(0,\infty)$. It is a notice that $f_i^{\downarrow}$ is strictly decreasing on $(0, f'_i(\gamma_i))$, while $f_i^{\uparrow}$ is strictly increasing on the same domain.

For $k=8$, define 
\[
F^{(k)}_i(\alpha)=\left\{\begin{matrix}
f_i(f_i^{\downarrow}(\alpha))   & \text{if}\quad G^{(k)}_i(\alpha)  \in I_i\\ 
0 & \text{if} \quad G^{(k)}_i(\alpha)  \not\in I_i
\end{matrix}\right.
\]
where $G^{(k)}_i(\alpha)=f_i^{\downarrow}(\alpha)$. The functions $F^{(9)}_i(\alpha)$ and $G^{(9)}_i(\alpha)$ are defined in a similar way, except that $f_i^{\downarrow}(\alpha)$ is replaced by $f_i^{\uparrow}(\alpha)$. Note that $\alpha=f'_i(x_i^{\text{R}})\le \max\{f'_i(\underline\xi_i),f'_i(\overline\xi_i),?\}$.

\noindent{\bf Case 9: (II) $\wedge$ (IV) $\wedge$ (VII)}. It follows from (\ref{dependC}) and (\ref{dependR}) that
\[
f'_i(x_i^{\text{R}})=g'_i(x_i^{\text{C}}) = \alpha.
\]
Since $g'_i$ is a one-to-one mapping, its inverse function exists and we have $x_i^{\text{C}}=(g'_i)^{-1}(\alpha)\equiv g_i^*(\alpha)$. 
We define
\[
G^{(k)}_i(\alpha)=f_i^{\downarrow}(\alpha)  + g_i^*(\alpha),
\]
and, 
\[
F^{(k)}_i(\alpha)=\left\{\begin{matrix}
f_i(f_i^{\downarrow}(\alpha))  + g_i(g_i^*(\alpha)),  & \text{if}\quad G^{(k)}_i(\alpha)\in I_i\\ 
0,&  \quad \text{otherwise},
\end{matrix}\right.
\]
for $k=10$. Similarly, we can define functions $F^{(11)}_i(\alpha)$ and $G^{(11)}_i(\alpha)$ by using $f_i^{\uparrow}(\alpha)$ instead of $f_i^{\downarrow}(\alpha)$.


Let $M=11$, and consider the following binary linear programming (BLP[$\alpha$]):
\begin{align}
\text{maximize}\quad &~  {\sum}_{i=1}^{N} \left\{ {\sum}_{k=1}^{M} y_{ik} \cdot F^{(k)}_i(\alpha)\right\} \quad {}&\\
\text{s.t.} \quad  &~ {\sum}_{i=1}^{N} \left\{ {\sum}_{k=1}^{M} y_{ik} \cdot G^{(k)}_i(\alpha)\right\} \le B, \label{res-constr} \\
&~ \sum_{k=1}^{M} y_{ik}=1,~\text{for}~ i\in [N]\\
&~ y_{ik}\in\{0,1\},~\text{for}~ i\in [N],
\end{align}   

\begin{lemma}
FSA is equivalent to BLP$[\alpha^*]$ in the sense that an optimal solution to the latter problem corresponds to an optimal allocation to the former one and vice versa.
\end{lemma}
\begin{proof}
Let $\alpha^*$ be the optimal Lagrange multiplier 
\end{proof}

The relaxation version of BLP, denoted by LP$[\alpha]$, is obtained by replacing binary variables by continuous ones in the domain $[0,1]$. It is noted that the functions $F^{(k)}_i(\alpha)$ and $G^{(k)}_i(\alpha)$ independent of $\alpha$ for $k\le 6$. Furthermore, it has been shown that the optimal Lagrange multiplier $\alpha$ is at most $\alpha_{\max}$, where
\[
\alpha_{\max}={\max}_{i\in[N]}\{f'_i(\underline\xi_i),f'_i(\overline\xi_i),g'_i(\underline\xi_i),f'_i(\gamma_i)\}.
\]
 Recall that $\gamma_i$ is the inflection point of $f_i$. Define $\Phi^{\text{LP}}:(0,\alpha_{\max}]\rightarrow \mathbb{R}$ the mapping that maps each positive value of $\alpha$ to an optimal objective value of the corresponding LP$[\alpha]$. We can define $\Phi^{\text{BLP}}:(0,\alpha_{\max}]\rightarrow \mathbb{R}$ in a similar way.



\begin{lemma}
An optimal solution $\alpha^{\text{LP}}$ of the univariate function $\Phi^{\text{LP}}$ can be found in polynomial time.
\end{lemma}
\begin{proof}
We claim that: i) $\Phi^{\text{LP}}$ is a univariate function that has a bounded number of discontinuous points; and ii) its maximizer can be found efficiently. Fixing $i\in[N]$. Regarding the first claim, it suffices to look at points $\alpha$ at which the functions $F^{(k)}_i$ and $G^{(k)}_i$ are discontinuous. One need to consider the cases when $7\le k\le 11$. 

\begin{itemize}
\item The function $G^{(7)}_i$ continuous, while $F^{(7)}_i$ is discontinuous at points $\alpha$ such that $g_i^*(\alpha)=\overline\xi_i$ or $g_i^*(\alpha)=\underline\xi_i$. Since $g_i^*$ is decreasing, there are exactly two values of $\alpha$ satisfying these two equations, and such values can be found efficiently. 
\item Consider the case $k=8$:  $G^{(8)}_i$ (and so $F^{(8)}_i$) may be discontinuous at $\alpha=\gamma_i$. In addition, $F^{(8)}_i$ is discontinuous at points $\alpha$ such that $f_i^{\downarrow}(\alpha)=\underline\xi_i$ or $f_i^{\downarrow}(\alpha)=\overline\xi_i$. Since, $f_i^{\downarrow}$ is strictly decreasing, there are at most two values of $\alpha$ satisfying, respectively, these two equalities. Similarly, we can give a same claim for the case of $G^{(9)}_i$ and $F^{(9)}_i$. Hence, the total number of possible discontinuous points of $F^{(8)}_i$ is $5$.
\item Consider the case $k=11$: we prove that the set of values of $\alpha$ such that $G^{(11)}_i(\alpha)\in I_i$ can be written as the union of at most two disjoint intervals, implying that the number of possible discontinuous points of $F^{(11)}_i$ is at most $5$: one for each endpoint of the intervals, plus one point that is the possible discontinuous point of  $G^{(11)}_i$. In order to show this, it suffices to prove that each of the two equations $G^{(11)}_i(\alpha)=\underline\xi_i$ and $G^{(11)}_i(\alpha)=\overline\xi_i$ has at most two roots. Indeed, if $\alpha>\gamma_i$ then $G^{(11)}_i(\alpha)=g_i^*(\alpha)$ and become a strictly decreasing function, and thus  the claim is easily followed. We consider case when $\alpha\le \gamma_i$. Consider the solution of the derivative of $(G^{(11)}_i)'$, which is obtained by solving the following equation:
\[
(f_i^{\uparrow})'(\alpha)  + (g_i^*)'(\alpha)=0\Leftrightarrow (f_i^{\uparrow})'(\alpha)  =- (g_i^*)'(\alpha).
\]
Since $(g'_i)^{-1}$ is differentiable on $\mathbb{R}_+\setminus\{0\}$, by using the formula for the derivative of an inverse function \cite{GS17}, we have
\begin{align*}
((g'_i)^{-1})'(\alpha)=&~\dfrac{1}{g''_i((g'_i)^{-1}(\alpha))}\\
=&~ - (g'_i)^{-1}(\alpha)\cdot ((g'_i)^{-1}(\alpha)+1)^2
\end{align*}
Hence,
\begin{equation}
\label{eq:fi-gi-1}
(f_i^{\uparrow})'(\alpha)  = (g'_i)^{-1}(\alpha)\cdot ((g'_i)^{-1}(\alpha)+1)^2
\end{equation}
The function on the left hand side of Eq. (\ref{eq:fi-gi-1}) is increasing, while the one on the right hand side is decreasing. Therefore the equation has at most one solution, meaning that $G^{(11)}_i$ has at most one local minimum, says $\hat \alpha$. One can see that $G^{(11)}_i$ is strictly decreasing on the interval $(0,\hat \alpha)$ and strictly increasing on the interval $(\hat \alpha,\gamma_i)$.  This follows that the number of roots of the  equation $G^{(11)}_i(\alpha)=c$ is at most $2$, for any $c>0$.

For the case of $F^{(10)}_i$, note that $G^{(11)}_i$ is deceasing function as it is sum of the two decreasing functions $f_i^{(1)}$ and $g_i^*$. Hence, the equation $G^{(10)}_i(\alpha)= c$ has at most one root for any $c>0$. Hence, the set $\{\alpha|G^{(10)}_i(\alpha)\in I_i\}$ is identical to  an interval $(a,b)$, where $a,b$ are respective the roots of $G^{(10)}_i(\alpha)= \overline\xi_i$ and of $G^{(10)}_i(\alpha)= \underline\xi_i$. In this case, the number of possible discontinuous points of $F^{(10)}_i$ is $3$.
\end{itemize}
We have proved that the set of discontinuous points of functions $F^{(k)}_i$ for $k\in[M]$ is a constant, for any $i\in[N]$, implying that $\Phi^{\text{LP}}$ has at most $O(N)$ discontinuous points. Let denote this set by $S=\{\alpha_t\}_{t=1,\ldots,T}$, where $\alpha_1<\alpha_2<\ldots<\alpha_T$. Then
\begin{equation}
\label{eq:maximize-phi-lp}
\max_{\alpha\in(0,\alpha_{\max}]} \Phi^{\text{LP}}(\alpha) = \max_{t=0}^T \left\{\Phi^{\text{LP}}(\alpha_t),\max_{\alpha\in (\alpha_t,\alpha_{t+1})} \Phi^{\text{LP}}(\alpha)\right\}, 
\end{equation}
where $\alpha_{T+1}=\alpha_{\max}$. It is noted that finding a maximizer of a  function $\Phi^{\text{LP}}$ that is continuous over an interval  $(\alpha_t,\alpha_{t+1})$ can be done by using bisection technique. Finally,
\[
\alpha^{\text{LP}} = \arg\max_{\alpha\in(0,\alpha_{\max}]} \Phi^{\text{LP}}(\alpha). 
\]
To solve (\ref{eq:maximize-phi-lp}), one needs to find a maximizer of  $\Phi^{\text{LP}}(\alpha)$ over the interval $(\alpha_t,\alpha_{t+1})$, for each $t\in T$, and this procedure takes at most $O(\log \max_i \{f_i,g_i\})$. Overall, (\ref{eq:maximize-phi-lp}) can be solved in $O(N\cdot \log \max_i \{f_i,g_i\})$ times.~\end{proof}

\begin{lemma}
Let $W$ be the value of the allocation returned by Algorithm~\ref{ptas}. The, it holds that  $W \ge (1-\epsilon)\cdot OPT^{\text{BLP}[\alpha^*]}$.
\end{lemma}
\begin{proof}
We first prove that
\begin{equation}
\label{eq:factor-approx}
W \ge (1-\epsilon)\cdot  OPT^{\text{LP}[\alpha^\text{LP}]}
\end{equation}

By the definition of BLP$[\alpha]$ and LP$[\alpha]$ and we have that
\begin{equation}
\label{eq:relationship}
OPT^{\text{LP}[\alpha^\text{LP}]}\ge OPT^{\text{LP}[\alpha^*]}\ge OPT^{\text{BLP}[\alpha^*]} 
\end{equation}

From (\ref{eq:factor-approx}) and (\ref{eq:relationship}) it follows the claim in the lemma.
\end{proof}

\begin{lemma}
One can find a solution to BLP$[\alpha^{\text{LP}}]$, whose value is at least a factor of $1-\epsilon$ of the optimum.
\end{lemma}
\begin{proof}

\end{proof}

\begin{algorithm}[!htb]
	\caption{{\bf PTAS}($\epsilon)$} \label{ptas}
\begin{algorithmic}[1]
%\Require Utility functions $u_i$, $i\in[N]$, the bandwidth capacity $B$, and an accuracy parameter $\epsilon>0$
%\Ensure A solution $\hat \cB$
\State Computing a maximizer $\bar \alpha$ of $\Phi^{\text{LP}}$ using bisection
 %{\Comment \em Finding a solution to BLP$[\bar \alpha]$}
%\For{each subset $U\subseteq [N]$ of size at most $1/\epsilon$}
%      \For{each subset $U\subseteq [N]$ of size at most $1/\epsilon$}     
%          \State $y_{ik}\leftarrow 1$ and    $y_{ik'}\leftarrow 0$ for $k'\not=k$
\State Guessing the set of at most $1/\epsilon$ users of highest utility
\State Finding an optimal BFS $\bf y$ to   LP$[\bar \alpha]$ %\label{step:scale}
\State Rounding down $\bf y$ to an integer solution $\bar {\bf y}$.
%\label{dyn}
\State Converting $\bar {\bf y}$ into an allocation;%\label{halt}
\State Allocate (remaining) bandwidth to an arbitrary user. %\label{kvalue}
%      \EndFor
%\EndFor
\end{algorithmic}
\end{algorithm}

==> reduction.tex <==
%\subsection{A reduction to multiple-choice knapsack}


\begin{proof}
We show a reduction to multiple-choice knapsack. We assume that the given instance of problem FSA is feasible. Furthermore, since the utility functions are increasing, we may assume without loss of generality that the equality in (\ref{capacity-constr}) is replaced by a "$\leq$". We also assume without loss of generality that $\overline\xi_i\le B$ for all $i$.
\subsubsection{Continuous case}
All variables $B_i^C$ and $B_i^R$ (and hence $B_i$) assume continuous values between $\underline \xi_i$ and $\overline \xi_i$.  
\subsubsection{Discrete case}
All variables $B_i^C$ and $B_i^R$ (and hence $B_i$) assume continuous values between $\underline \xi_i$ and $\overline \xi_i$.

\noindent{\it Lower bounding OPT.} First we derive a {\it positive} lower bound $L$ on the value of the optimum solution. If $\underline\xi_i=0$ for all $i$, then $L:=\max_i u_i(\min\{\overline\xi_i,B\})>0$ is a lower bound on OPT. Otherwise, (by feasibility of the instance) $L:=\sum_iu_i(\underline\xi_i)>0$ is a lower bound on OPT.

\noindent{\it Discretization.} 
For each $i\in[N]$, define $f_i^j:=\frac{\epsilon L}{N}(1+\epsilon)^j$, for $j=-\infty,0,1\ldots,K_f:=\left\lceil\log_{(1+\epsilon)}\frac{Nf_i(\overline\xi_i)}{\epsilon L}\right\rceil$. As $f_i(\cdot)$ is strictly monotone increasing, the equation $f_i(x)=f_i^j$, for $j=0,1,\ldots,K_f$, has a unique positive root $x_i^j$ in the interval $[0,\overline\xi_i]$. Given any desired accuracy $\epsilon_0>0$, we can approximate this root to within an absolute error of $\epsilon_0$ using the bisection method:
\begin{align}\label{approx-root}
|\tilde x_i^j-x_i^j|\le\epsilon_0,
\end{align}
in time $O(\log \frac{f_i(\overline\xi_i)}{\epsilon_0})$, where $\tilde x_i^j$ denotes the approximate root. We need to pick $\epsilon_0$ small enough such that 
\begin{align*}
|f_i(\tilde x_i^j)-f_i(x_i^j)|\le\epsilon  f_i(x_i^j),
\end{align*}
which would imply that
\begin{align}\label{approx-f}
f_i(\tilde x_i^{j})\le f_i(x)\le \frac{(1+\epsilon)^2}{1-\epsilon}f_i(\tilde x_i^j),
\end{align}
for all $j=0,1,\ldots,K_f-1$ and $x\in[\tilde x_i^{j},\tilde x_i^{j+1}]$. (To see this, note that $x\in[\tilde x_i^j,\tilde x_i^{j+1}]$ implies that
\begin{align*}
f_i(\tilde x_i^{j})\le f_i(x)\le f_i(\tilde x_i^{j+1}).
\end{align*}
Combining this with (\ref{approx-f}), we get
\begin{align*}
f_i(x)&\le (1+\epsilon)f_i(x_i^{j+1})=(1+\epsilon)(1+\epsilon)^{j+1}\frac{\epsilon L}{N}\\
&=(1+\epsilon)^2f_i(x_i^j)\le \frac{(1+\epsilon)^2}{1-\epsilon}f_i(\tilde x_i^j).)
\end{align*}
Recall that a continuous function $f:\mathbb{R}\to\mathbb{R}$ is $c$-Lipschitz  if for all $x$ and $x'$ (in the domain of $f$), $|f(x)-f(x')|\le c|x-x'|$, and a sufficient condition for this is that $|f'(x)|\le c$ for all $x$. Using the definition of $f_i$, 
\begin{align*}
f'_i(x)= \frac{\nu_i\delta}{T_p}\cdot \dfrac{x}{1+\nu_i x^2}\le \frac{\sqrt\nu_i\delta}{2T_p}.
\end{align*}
It follows that we should select $\epsilon_0:=\frac{2T_p\epsilon^2L}{\sqrt\nu\delta N}$, so that
\begin{align*}
|f_i(\tilde x_i^j)-f_i(x_i^j)|\le\frac{\sqrt\nu_i\delta}{2T_p}|\tilde x_i^j-x_i^j|\le \epsilon f_i(x_i^j).
\end{align*}
%$\epsilon_0:=\min\left\{\frac{2T_p\epsilon^2L}{\sqrt\nu\delta N},\frac12\right\}$

Similarly, for each $i\in[N]$, define $g_i^j:=\frac{\epsilon L}{N}(1+\epsilon)^j$, for $j=-\infty,0,1\ldots,K_g:=\left\lceil\log_{(1+\epsilon)}\frac{Ng_i(\overline\xi_i)}{\epsilon L}\right\rceil$. Again, $g_i(\cdot)$ is strictly monotone increasing, and hence the equation $g_i(x)=g_i^j$, for $j=0,1,\ldots,K_g$, has a unique positive root $y_i^j$ in the interval $[0,\overline\xi_i]$. Let  $\tilde y_i^j$ be an approximation of this root to within an absolute error of $\epsilon_0$, which can be obtained by the bisection method in time $O(\log \frac{g_i(\overline\xi_i)}{\epsilon_0})$. Note however that $g_i'(0)=\infty$ and thus, in order to use a similar argument as above, we need first to restrict $g_i$ to an interval that is sufficiently away from $0$. Let $c_i>1$ be a constant that will be determined later and $y_0:=\frac{\epsilon L}{c_iN}$. Then, 
\begin{align*}
g_i(y_0)=\frac{\epsilon L}{cN}\log\left(1+\dfrac{c_iN\tau_i}{\epsilon L}\right).
\end{align*}
If $\dfrac{N\tau_i}{\epsilon L}\le e$, then $c_i=2$ would give $g_i(y_0)\le\frac{\epsilon L}{N}\cdot\frac{\log (1+2e)}{2}<\frac{\epsilon L}{N}$. Otherwise, let $c_i=e\log \frac{N\tau_i}{\epsilon L}$. Then
\begin{align*}
g_i(y_0)&\le\frac{\epsilon L}{c_iN}\log\left((1+c_i)\dfrac{N\tau_i}{\epsilon L}\right)=\frac{\epsilon L}{N}\left(\frac{\log(1+c_i)}{c_i}+\frac{1}{e}\right)\\&<\frac{\epsilon L}{N},
\end{align*}
using the inequality $\log(1+ea)<(e-1)a$, valid for all $a\ge1$. In both cases we get that $g_i(y_0)< \frac{\epsilon L}{N}$, and thus by monotonicity, the root $y_i^1$ (at which $g_i(y_i^1)=\frac{\epsilon L}{N}$) lies in the interval $[y_0,\overline\xi_i]$. Now, for any $x$ in this interval
\begin{align*}
g'_i(y)&=  \log\left(\dfrac{\tau_i+x}{x}\right)-\dfrac{\tau_i}{\tau_i+x}\\&\le\log\left(\dfrac{\tau_ic_iN}{\epsilon L}+1\right)\le \dfrac{\tau_ic_iN}{\epsilon L}.
\end{align*}
Then we need to pick $\epsilon_0:=\frac{\epsilon^3 L^2}{N^2\tau_ic_i}$, so that 
\begin{align*}
|g_i(\tilde y_i^j)-g_i(y_i^j)|\le\dfrac{\tau_ic_iN}{\epsilon L}|\tilde y_i^j-y_i^j|\le \epsilon g_i(x_i^j),
\end{align*}
which gives
\begin{align}\label{approx-g}
g_i(\tilde y_i^{j})\le g_i(y)\le \frac{(1+\epsilon)^2}{1-\epsilon}g_i(\tilde y_i^j),
\end{align}
for all $j=0,1,\ldots,K_g-1$ and $y\in[\tilde y_i^{j},\tilde y_i^{j+1}]$.

It is easy to see from the above discussion that such discretization can be done in time linear in the maximum bit length $\cL$ of the input parameters (such as $N$, $\nu_i$, $\tau_i$, $f_i(\overline \xi_i)$, etc).


\noindent{\it The multiple-choice knapsack problem (MCKP).} Recall that in MCKP, we are given a set of $N$ users, with a discrete demand set $D_i$ for each user $i$, and a utility function $U_i:D_i\to\mathbb{R}_+$, giving the utility enjoyed by user $i$ if her/his demand $d_i\in D_i$ is fulfilled. Given a bound $B$ on the total demand, the objective is to choose a demand $d_i\in D_i$ for each user, so as to maximize $\sum_iU_i(d_i)$ subject to $\sum_id_i\le B$. 

We can model the discretized version of FSA as an MCKP as follows. For user $i$, we define 
\[
D_i^x:=\big\{\tilde x_i^j\big\}_j\cup\{0,\underline\xi_i,\overline\xi_i\},
\]
and
\[
D_i^y:=\big\{\tilde y_i^j\big\}_j\cup\{\underline\xi_i-\tilde x_i^j:~\tilde x_i^j<\underline\xi_i\}_j\cup\{0,\underline\xi_i,\overline\xi_i\},
\]
Let $D_i:=D_i^x\times D_i^y$, and for $d_i=(d_i^x,d_i^y)\in D_i$ define
\begin{align*}
U_i(d_i)&:=\left\{\begin{array}{ll}
f_i(d_i^x)+g_i(d_i^y)&\text{if }\underline\xi_i\le d_i^x+d_i^y\le\overline\xi_i\\
-\infty&\text{otherwise}.
\end{array}
\right.
\end{align*}
Given an optimal solution $\{(x_i^*,y_i^*)\}_i$ for FSA:
\begin{align*}
\text{OPT}=\sum_i(f_i(x_i^*)+g_i(y_i^*))\\
\sum_{i}(x_i^*+y_i^*)\le B\\
\underline\xi_i\le x_i^*+y_i^*\le\overline\xi_i,\quad\forall i,
\end{align*}
 we show that MCKP has a feasible solution $\{(d_i^x,d_i^y)\}_i$ with $\sum_iU_i(d_i)\ge (1-O(\epsilon))\text{OPT}$. 
 
% We first obtain a modified solution $\{(x_i',y_i')\}_i$ as follows. If $f_i(x_i^*)<\frac{\epsilon L}{N}$ (resp., $g_i(y_i^*)<\frac{\epsilon L}{N}$), set $x_i':=0$ and $y_i':=x_i^*+y_i^*$ (resp., $x_i':=0$ and $y_i':=x_i^*+y_i^*$). (If both conditions $f_i(x_i^*)<\frac{\epsilon L}{N}$ and $g_i(y_i^*)<\frac{\epsilon L}{N}$ hold, we set $x_i':=0$ and $y_i':=x_i^*+y_i^*$.) Note that $\{(x_i',y_i')\}_i$ is still feasible, and $\sum_i(f_i(x_i')+g_i(y_i'))\ge (1-\epsilon)\text{OPT}$ as the total loss in utility is at most $\frac{\epsilon L}{N}\cdot N\le \epsilon \text{OPT}$.
 Let $\bar d_i^x$ (resp., $\bar d_i^y$) be the largest element in $\{\tilde x_i^j\}_j$ (resp., $\{\tilde y_i^j\}_j$) such that $\bar d_i^x\le x_i^*$ (resp., $\bar d_i^y\le y_i^*$). 
We define the solution $\{(d_i^x,d_i^y)\}_i$ to MCKP as follows: 
 \begin{align*}
d_i^x&:=\bar d_i^x\\
d_i^y&:=\left\{
\begin{array}{ll}
\underline\xi_i-\bar d_i^x&\text{if }\bar d_i^x+\bar d_i^y<\underline \xi_i\\
\bar d_i^y&\text{otherwise.}
\end{array}
\right.
 \end{align*}
 Note that this gives a solution to MCKP with finite utility.
Let $J^x$ (resp., $J^y$) be the set of customers $i$ such that $f_i(x_i^*)\ge \frac{\epsilon L}{N}$ (resp., $g_i(y_i^*)\ge \frac{\epsilon L}{N}$). Then by (\ref{approx-f}) (resp., (\ref{approx-g})), for any $i\in J^x$ (resp., $i\in J^y$), we have
$f_i(\bar d_i^x)\ge\frac{(1-\epsilon)}{(1+\epsilon)^2}f_i(x_i^*)$ (resp., $g_i(\bar d_i^y)\ge\frac{(1-\epsilon)}{(1+\epsilon)^2}g_i(y_i^*)$). 
On the other hand, $\sum_{i\not\in J^x}f_i(x_i^*)+\sum_{i\not\in J^y}g_i(y_i^*)\le 2\frac{\epsilon L}{N}\cdot N\le 2\epsilon\cdot\text{OPT}$.
  It follows that
\begin{align*}
\sum_iU_i(d_i)&:=\sum_i(f_i(d_i^x)+g_i(d_i^y))\ge\sum_i(f_i(\bar d_i^x)+g_i(\bar d_i^y))\\
&\ge\frac{(1-\epsilon)}{(1+\epsilon)^2}\left(\sum_{i\in J^x}f_i(x_i^*)+\sum_{i\in J^y}g_i(y_i^*)\right)\\
&\ge\frac{(1-\epsilon)(1-2\epsilon)}{(1+\epsilon)^2}\text{OPT}.
\end{align*} 


\subsection{The discrete case}

\noindent{\it Dealing with the discrete case.} The above reduction works for the continuous case. With a slight modification, it can also be used to deal with the discrete case. Namely, we define $D_i^x:=\big\{\lfloor\tilde x_i^j\rfloor,\lceil\tilde x_i^j\rceil\big\}_j\cup\{0,\underline\xi_i,\overline\xi_i\}$, $D_i^y:=\big\{\lfloor\tilde y_i^j\rfloor,\lceil\tilde y_i^j\rceil\big\}_j\cup\{\underline\xi_i-\lfloor\tilde x_i^j\rfloor:~\lfloor\tilde x_i^j\rfloor<\underline\xi_i\}_j\cup\{\underline\xi_i-\lceil\tilde x_i^j\rceil:~\lceil\tilde x_i^j\rceil<\underline\xi_i\}_j\cup\{0,\underline\xi_i,\overline\xi_i\}$. 
Given an optimal solution $\{(x_i^*,y_i^*)\}_i$ for FSA, we define the corresponding solution of MCKP as follows. Let $\bar d_i^x$ (resp., $\bar d_i^y$) be the largest element in $\big\{\lfloor\tilde x_i^j\rfloor,\lceil\tilde x_i^j\rceil\big\}_j$ (resp., $\big\{\lfloor\tilde y_i^j\rfloor,\lceil\tilde y_i^j\rceil\big\}_j$) such that $\bar d_i^x\le x_i^*$ (resp., $\bar d_i^y\le y_i^*$). Then we define $d_i^x$ and $d_i^y$ as in the continuous case.
For the rest of the  argument to go through, it is enough to verify that $f_i(\bar d_i^x)\ge\frac{(1-\epsilon)}{(1+\epsilon)^2}f_i(x_i^*)$ (resp., $g_i(\bar d_i^y)\ge\frac{(1-\epsilon)}{(1+\epsilon)^2}g_i(y_i^*)$). This is easily shown as follows. Suppose that $x_i^*\in[\tilde x_i^j,\tilde x_i^{j+1}]$. Then $\bar d_i^x\in\big\{\lfloor\tilde x_i^j\rfloor,\lceil\tilde x_i^j\rceil\big\}$. If $\bar d_i^x=\lceil\tilde x_i^j\rceil$ then by (\ref{approx-f}), $f_i(\bar d_i^x)\ge f_i(\tilde x_i^j)\ge \frac{(1-\epsilon)}{(1+\epsilon)^2}f_i(x_i^*)$. Otherwise, $\lfloor\tilde x_i^j\rfloor\le x_i^*< \lceil\tilde x_i^j\rceil$ implies by the integrality of $x_i^*$ that $x_i^*=\lfloor\tilde x_i^j\rfloor$ and hence $f_i(\bar d_i^x)=f_i(x_i^*)$. A similar argument can be used to show that $g_i(\bar d_i^y)\ge\frac{(1-\epsilon)}{(1+\epsilon)^2}g_i(y_i^*)$.~\end{proof}
